Equivelar toroids with few flag-orbits

An $(n+1)$-toroid is a quotient of a tessellation of the $n$-dimensional Euclidean space with a lattice group. Toroids are generalizations of maps in the torus on higher dimensions and also provide examples of abstract polytopes. Equivelar toroids are those that are induced by regular tessellations. In this paper we present a classification of equivelar $(n+1)$-toroids with at most $n$ flag-orbits; in particular, we discuss a classification of $2$-orbit toroids of arbitrary dimension.

==> norbit.tex <==
\subsubsection{Cubic $(n+1)$-toroids with $n$ flag-orbits}

Now we proceed to classify $(n+1)$-cubic toroids with $n$ flag-orbits for $n \geq 4$. The strategy is essentially the same that we have use before: first we determine the $n$-index subgroups of $\stabcube$ and then we determine the lattices preserved by each of them. In order to classify $n$-index subgroups of $\stabcube$ we need the following result regarding permutation groups, which is a consequence of \cite[Theorem 5.2B]{dixonPermutationGroups}.

\begin{thm}\label{thm:indexnSubgpsSn}
 Let $n \geq 5$ and $S_{n}$ the group of permutations of $\{1, \dots , n \}$. If $G$ is an index-$n$ subgroup of $S_{n}$ then up to conjugacy, one of the following holds:
 \begin{itemize}
  \item The group $G$ is the stabilizer of $\{n\}$ and hence, isomorphic to $S_{n-1}$.
  \item $n = 6$ and $G$ acts on $\{1, 2, \dots 6\}$ as the group $PGL_{2}(5)$ acts on the points of the projective plane over $\bF_{5}$, the field with $5$ elements. 
 \end{itemize}
\end{thm}

Now we may classify index-$n$ subgroups of $\stabcube$.

\begin{lem}\label{lem:cubicIndexnSubgps}
 Let $n \geq 4$. If $K$ is an index-$n$ subgroup of $\stabcube$, then up to conjugacy one of the following holds:
 \begin{itemize}
  \item $K = \abeln \rtimes \symn[n-1]$.
  \item $n = 4$ and $K = \abeln[4] \rtimes \altn[4]$.
  \item $n=6$ and $K=\abeln[6] \rtimes \pgl$.
 \end{itemize}
	Here $\symn[n-1]$ denotes the stabilizer of the last coordinate in $\symn$ and $\pgl$ denotes the subgroup of $\symn[6]$ that acts on the coordinates of $\E[6]$ as $PGL_{2}(5)$.
 \begin{proof}
  The result is a consequence of Theorem\nobreakspace \ref {thm:indexnSubgpsSn}. By Equation\nobreakspace \textup {(\ref {eq:indexIm})}, $[\symn:\eta(K)] \leq n$, which implies that $\eta(K)$ is $\symn$, $\altn$, or one of the group described in Theorem\nobreakspace \ref {thm:indexnSubgpsSn}. Let $K_{0} = K \cap \abeln$ and recall that $|K|= |\eta(K)||K_{0}|$. 
  
  If $\eta(K) = \symn$, then $|K| = (n-1)! 2^{n} = n! |K_{0}|$, which implies that $\frac{2^{n}}{n}= |K_{0}|$. However, if $n \geq 4$ we have $2 < \frac{2^{n}}{n} < 2^{n-1}$ but this is impossible since $K_{0}$ is a subgroup of $\abeln$ normalized by $\symn$ and by Lemma\nobreakspace \ref {lem:preservedByAn}, must be one among $\abeln$, $\abelnplus$ and $\minid$.
  
  Proceeding in an analogous way we may see that if $\eta(K) = \altn$, the unique possibility for $K_{0}$ is $\abelnplus$ and this is only possible if $n=4$. With similar arguments to that used the proof of Lemma\nobreakspace \ref {lem:index2Cube} we may conclude that $K = \altn[4] \rtimes \abelnplus[4]$.
  
  Finally, if $\eta(K)$ has index $n$ in $\symn$, then we have $|K| = (n-1)! 2^{n} = |\eta(K)| |K_{0}|=(n-1)! |K_{0}|$, therefore $K_{0}$ must be $\abeln$ and $K = \abeln \rtimes \symn[n-1]$ or $n=6$ and $K= \abeln \rtimes \pgl$. 
 \end{proof}
\end{lem}

Now we proceed to classify lattices preserved by index-$n$ subgroups of $\stabcube$. Lattices preserved by $\abelnplus[4] \rtimes \altn[4]$ are described in Lemma\nobreakspace \ref {lem:laticesC2plusAlt}. It only remains to determine those rank-$n$ lattices preserved by $\abeln \rtimes \symn[n-1]$ and those rank-$6$ lattices preserved by $\abeln[6] \rtimes \pgl$. Such lattices are described in the following results.

\begin{lem}\label{lem:latticesPGL25}
	If $\LL$ is an integer rank-$6$ lattice preserved by $\abeln[6] \rtimes \pgl$, then $\LL = s \regLat[6]$ for some $s \in \bZ$ and $k \in \{1,2,6\}$. 
	\begin{proof}
		Let $\LL$ be a rank-$6$ lattices preserved by $\abeln[6] \rtimes \pgl$. Let $s \in \bZ$ a positive integer such that every entry of any vector in $\LL$ has absolute value at least $s$. As before, this implies that the entries of any vector of $\LL$ are multiples of $s$. Let $(s_{1}, \dots , s_{6}) \in \LL$. Given the transitive action of $\pgl$ on the coordinates of $\E[6]$, we may assume that $s_{1} = s$. Since $\LL$ is preserved by $\abeln[6]$ this implies that $(-s,s_{2},\dots,s_{6}) \in \LL$. Hence $2s e_{1} \in \LL$ and therefore $2s e_{i} \in \LL$ for $i \in \{1, \dots , 6\}$. 
		
		We may take $(s_{1}, \dots , s_{6}) \in \bLL$ whose all entries are either $0$ or $s$. Furthermore, since the action of $\pgl$ is $3$-transitive on the coordinates of $\E[6]$, we may assume that $(s_{1}, \dots , s_{6})$ is of the form $(s^{k},0^{6-k})$. Among all non-zero points in $\LL$ with this form take one of those where $k$ is minimum.  
		
		If $k =1$ then $se_{i} \in \LL$ for $i \in \{1, \dots,6\}$ which implies that $\cln[5] \subset \LL$. However, since all the vectors of $\LL$ have integer entries multiples of $s$, we must have $\LL = \cln[5]$.
		
		Suppose $k=2$. Since $\LL$ is preserved by $\pgl$, then $\fcln[4] \subset \LL$. On the other hand, by the observations made above every point of $\LL$ may be written as the sume of  a point in $\fcln[4]$ and a point in $2s\cln[5]$. Since  $2s\cln[5] \leq \fcln[4]$ we must have $\LL \subset \fcln[4]$. 
		
		Suppose $k \in \{3,4,5\}$ and take $(s^{k}, 0 ^{6-k}) \in \LL$. Given that $\LL$ is preserved by $\pgl$, we must have that $(0, s^{k}, 0^{6-k-1})$ is a point of $\LL$. This implies that $(s,0,0,0,0,s) \in \LL$, hence $(s,s,0,0,0,0) \in \LL$ which contradicts the choice of $k$.
		
		Finally, if $k = 6$ proceding by an analogous way of that used when $k=2$, we may conclude that $\LL = s \bcln[6]$.
	\end{proof}
\end{lem}

The previous lemma implies that all $(6+1)$-toroids induced by lattices preserved by $\abeln[6] \rtimes \pgl$ are regular toroids. Since all $(4+1)$-toroids induced by lattices preserved by $\abeln[4] \rtimes \altn[4]$ are regular or $2$-orbit, Lemma\nobreakspace \ref {lem:cubicIndexnSubgps} implies that if there exist $(n+1)$-toroids with $n$ flag-orbits, they must be induced by lattices preserved by $\abeln \rtimes \symn[n-1]$ that do not induce regular toroids. We now proceed to classify those lattices.

We use Lemma\nobreakspace \ref {lem:refLattices} to classify lattices preserved by $\abeln \rtimes \symn[n-1]$. To set the context, we shall assume that $\symn[n-1]$ is precisely the stabilizer of the last coordinate on $\E$. Let $\Pi$ the plane $x_{n}=0$ and $R$ the reflection through $\Pi$, this is $R: (x_{1}, \dots , x_{n}) \mapsto (x_{1}, \dots, -x_{n})$. If $\LL$ is a lattice preserved by $\abeln \rtimes \symn[n-1]$, then $\LL$ is a lattice preserved by $R$. Since $\symn[n-1]$ preserves $\Pi$, if $\LL_{0}=\LL \cap \Pi$, then $\LL_{0}$ must be a rank-$(n-1)$ lattice preserved by the restriction of the action of $\abeln \rtimes \symn[n-1]$ to $\Pi$ and therefore $\LL_{0}$ must be one among $s_{0}\cln[n-2]$, $s_{0}\fcln[n-3]$ and $s_{0}\bcln[n-1]$ for some positive integer $s_{0}$. 

Assume that $\LL_{0} = s_{0}\cln[n-2]$. If $\LL$ is a vertical translation lattice then $\LL = \trasLat[(de_{n})] $ for some $d \in \bN$. If $d=s_{0}$ then $\LL = \cln$; in any other case $\LL$ is a lattice preserved by $\abeln \rtimes \symn[n-1]$. Since this group is maximal in $\stabcube$ and $\LL$ does not induce a regular toroid, then $\LL$ induce a $n$-orbit toroid.

Suppose that $\LL$ is not a vertical translation lattice. Let $u$ be the point of $\LL \cap \Pi^{\perp}$ closets to $o$, say $u= d e_{n}$.  By Lemma\nobreakspace \ref {lem:refLattices} there exist unique $\alpha_{1}, \dots, \alpha_{n-1} \in \{0,1\}$, not all zero, such that if $w=\frac{s_{0}}{2}\left(\alpha_{1}e_{1} + \cdots + \alpha_{n-1}e_{n-1}\right) + \frac{d}{2} e_{n} $, then $\LL = \trasLat$. Since $\LL$ is preserved by $\symn[n-1]$ the only possible choice of $\alpha_{1}, \dots, \alpha_{n-1}$ is $\alpha_{1}= \cdots= \alpha_{n-1}=1$. Since $w$ must be a point with integer coordinates, $s_{0}$ and $d$ must be even. If $d=s_{0}$, then $\LL = \frac{s_{0}}{2} \bcln$. In any other case $\LL$ induce an $n$-orbit toroid. 

Now assume that $\LL_{0} = s_{0} \fcln[n-3]$. If $\LL$ is a vertical translation lattice, then $\LL = \trasLat[(de_{n})]$ for some $d \in \bN$: In this case, any choice of $d$ gives a lattice preserved by $\abeln \rtimes \symn[n-1]$ that does not induce a regular toroid. Any such lattice must then induce an $n$-orbit toroid.

Assume $\LL$ is not a vertical translation lattice. Let $u$ be  the closest point of $\Pi^{perp}$ to $o$, say $u=de_{n}$ for some integer $d$. Recall that $\{2s_{0}e_{1}, s_{0}(e_{2}-e_{1}), s_{0}(e_{3}-e_{2}), \dots , s_{0}(e_{n-1}-e_{n-2})\}$ is a basis for $\LL_{0}$. Take $\alpha_{1}, \dots , \alpha_{n-1} \in \{0,1\}$, not all zero, such that 
\begin{align*}
	w &= \frac{s_{0}}{2} \Big( \alpha_{1} (2e_{1}) + \alpha_{2} (e_{2}-e_{1}) + \dots \alpha_{n-1}(e_{n-1}-e_{n-2}) \Big) + \frac{d}{2}e_{n}\\
	&=  \frac{s_{0}}{2} \Big( (2\alpha_{1}-\alpha_{2})e_{1} + (\alpha_{2}-\alpha_{3})e_{2}+ \cdots + (\alpha_{n-2}-\alpha_{n-1})e_{n-2} + \alpha_{n-1} e_{n-1}\Big)+ \frac{d}{2}e_{n}
\end{align*}
satisfies that $\LL = \trasLat $. Let $w_{i}$ be the image of $w$ under the reflection on the plane $x_{i}=0$ for $1 \leq i \leq n-1$. Since $\LL$ is preserved by $\abeln$, $w_{i} \in \LL$ for all $i \in \{1, \dots, n-1\}$. If $\alpha_{n-1}=1$ then $w - w_{n-1} = s_{0}e_{n-1}$. This contradicts that $\LL_{0} = s_{0} \fcln[n-3]$; then $\alpha_{n-1} = 0$. Similarly if $\alpha_{n-1} = 0$ and $\alpha_{n-2} = 1$, then $w - w_{n-1} = s_{0}e_{n-2}$, hence $\alpha_{n-2} =0$. Proceding in an analogous way, we may conclude that $\alpha_{2} = \cdots = \alpha_{n-1}=0$, which implies that $\alpha_{1}=1$ and $w= s_{0} e_{1} + \frac{d}{2} e_{n}$. Again, since $w$ must have integer coordinates, then $d$ must be even. If $d=s_{0}$, then $\LL = \fcln$. In any other case $\LL$ is a lattice that induce an $n$-orbit toroid.

Assume that $\LL_{0} = s_{0}\bcln[n-1]$. If $\LL$ is a vertical translation lattice, then $\LL = \trasLat[(de_{n})]$ for some $d \in \bN$. In this case, any choice of $d$ gives a lattice preserved by $\abeln \rtimes \symn[n-1]$ that induce a non-regular toroid. Those lattices must induce an $n$-orbit toroid.

If $\LL$ is not a vertical translation lattice with respecto to $\Pi$, as before, take $u \in \Pi^{\perp} \sm \{o\}$ closest to $o$, say $u=de_{n}$ for some $d \in \bN$. Since $\{2e_{1}, \dots , 2e_{n-2}, e_{1} + \cdots + e_{n-1}\}$ is a basis for $\LL_{0}$, by Lemma\nobreakspace \ref {lem:refLattices} there exist $\alpha_{1}, \dots, \alpha_{n-1}$ such that
\begin{align*}
	w &= \frac{s_{0}}{2} \Big( \alpha_{1} (2e_{1}) +  \dots + \alpha_{n-2}(2e_{n-2}) + \alpha_{n-1}(e_{1} + \cdots +e_{n-1}) \Big) + \frac{d}{2}e_{n}\\
	&=  \frac{s_{0}}{2} \Big( (2\alpha_{1}+\alpha_{n-1})e_{1} + \cdots + (2\alpha_{n-2}+\alpha_{n-1})e_{n-2}+   \alpha_{n-1} e_{n-1}\Big)+ \frac{d}{2}e_{n}
\end{align*}
satisfies that $\LL = \trasLat$. For $i \in \{1, \dots, n-1\}$ let $w_{i}$ the image of $w$ under the refelction on the plane $x_{i} = 0$. If $\alpha_{n-1} = 1$ then $w - w_{n-1} = s_{0} e_{n}$, which contradicts that $\LL_{0} = s_{0}\bcln$; then $\alpha_{n-1} = 0$. Let $i \in \{1, \dots, n-2\}$ such that $\alpha_{i} = 1$ and let $S_{i}$ the reflection $(x_{1}, \dots, x_{n}) \mapsto (x_{1}, \dots, x_{i-1}, x_{n-1}, x_{i+1}, \dots x_{n-2}, x_{i}, x_{n} )$, then $w-w_{i}S_{i} = s_{0}(e_{i} + e_{n-1})$ which for $n \geq 4$ does not belong to $s_{0} \bcln[n-1]$. This is a contradiction. Therefore if $\LL_{0} = s_{0} \bcln$, then $\LL$ must be a vertical translation lattice.

The previous discussion completes the classification of cubic toroids with $n$ flag-orbits. We sumarize such discussion in the following result.

% \begin{thm}\label{thm:n-orbit}
% 	Let $n \geq 4$. Every equivelar $n$-orbit toroid of rank $(n+1)$ may be described as a toroid $\{4, 3^{n-2}, 4\}_{\bLL}$ where $\bLL$ is the lattice group associated to one of the following lattices:
% 	\begin{enumerate}
% 		\item $\bigcup_{k \in \bZ} \left( s_{0} \cln[n-2] + k(de_{n}) \right)$ for some $s_{0}, d \in \bN$, $s_{0} \neq d$.
% 		\item $\bigcup_{k \in \bZ} \left( s_{0} \cln[n-2] + k(d(e_{1}+ \cdots e_{n})) \right)$ for some $s_{0}, d \in \bN$, $s_{0}$ and $d$ even, and $s_{0} \neq d$.
% 		\item $\bigcup_{k \in \bZ} \left( s_{0} \fcln[n-3] + k(de_{n}) \right)$ for some $s_{0}, d \in \bN$.
% 		\item $\bigcup_{k \in \bZ} \left( s_{0} \fcln[n-3] + k(d(e_{1}+ \cdots e_{n})) \right)$ for some $s_{0}, d \in \bN$, $s_{0}$ and $d$ even, and $s_{0} \neq d$.
% 	\end{enumerate}

% \end{thm}



